Joint Scheduling of URLLC and eMBB Traffic in 5G Wireless Networks

Emerging 5G systems will need to efficiently support both enhanced mobile broadband traffic (eMBB) and ultra-low-latency communications (URLLC) traffic. In these systems, time is divided into slots which are further sub-divided into minislots. From a scheduling perspective, eMBB resource allocations occur at slot boundaries, whereas to reduce latency URLLC traffic is pre-emptively overlapped at the minislot timescale, resulting in selective superposition/puncturing of eMBB allocations. This approach enables minimal URLLC latency at a potential rate loss to eMBB traffic. We study joint eMBB and URLLC schedulers for such systems, with the dual objectives of maximizing utility for eMBB traffic while immediately satisfying URLLC demands. For a linear rate loss model (loss to eMBB is linear in the amount of URLLC superposition/puncturing), we derive an optimal joint scheduler. Somewhat counter-intuitively, our results show that our dual objectives can be met by an iterative gradient scheduler for eMBB traffic that anticipates the expected loss from URLLC traffic, along with an URLLC demand scheduler that is oblivious to eMBB channel states, utility functions and allocation decisions of the eMBB scheduler. Next we consider a more general class of (convex/threshold) loss models and study optimal online joint eMBB/URLLC schedulers within the broad class of channel state dependent but minislot-homogeneous policies. A key observation is that unlike the linear rate loss model, for the convex and threshold rate loss models, optimal eMBB and URLLC scheduling decisions do not de-couple and joint optimization is necessary to satisfy the dual objectives. We validate the characteristics and benefits of our schedulers via simulation.

==> horizontal_vs_vertical-orig.tex <==
\subsection{Optimal eMBB Slot Aggregation}
\label{sec:eMBB_slot_aggregation}
In Sec.~\ref{sec:sys-model} we have used uniform slot sizes for eMBB users, i.e. the allocated minislots to all users span the entire width of the slot (see Figure~\ref{fig:config_2}). However, new proposals allow greater flexibility in slot allocation, e.g., the capability to choose different slot durations for different eMBB users~\cite{3gpp_ran1_87}.
% include aggregation of eMBB slots
% and coding across eMBB slots for a given eMBB user
% as well as the capability to choose different slot durations for different eMBB users~\cite{3gpp_ran1_87}.
An example of such an eMBB resource allocation configuration is shown in Fig.~\ref{fig:emBB_slots}.
%Note that in this figure eMBB users 1 and 2 are allocated resources for an eMBB slot duration  and eMBB user 3 is allocated resources for an aggregated slot by combining two eMBB slots.     

%In an eMBB slot, eMBB users can share resources in time or frequency. 
%If only time is shared among  eMBB users, the entire frequency is allocated to an eMBB user in a mini-slot. Similarly if only frequency resource are share  among eMBB users, then  a purceart of the bandwidth is allocated to an eMBB user for the entire eMBB slot. Sharing resources in the time and frequency domains are illustrated in Figures~\ref{fig:config_1} and~\ref{fig:config_2}, respectively.



Here we will justify the  use of uniform slot sizes for eMBB users in Sec.~\ref{sec:sys-model}. We  show that choosing a slot duration equal to a common \emph{coherence time}\footnote{In a wireless network, different users may have different channel coherence times due differences in user mobilities.  We take the minimum  of coherence times of eMBB  users} of eMBB users' channels  along with appropriate bandwidth allocations  results in a better average eMBB rate under minislot homogeneous URLLC placement policies. 

% This leads to resource allocations where  eMBB users use different parts of the spectrum for  different duration, for example, one such configuration is shown in Fig.~\ref{fig:emBB_slots}.  In addition to the efficient scheduling of eMBB users, next generation radio technologies have to support efficient multiplexing of URLLC and eMBB traffic via puncturing mechanisms. In this document we shall show that allocating different duration in the time domain for eMBB would result in higher losses in throughput for the eMBB users due to URLLC puncturing. 
\begin{figure}
	\centering
	\includegraphics[scale=0.35]{eMBB_flexibile_resource_allocation}
	\caption{An example of eMBB resource allocations in 5G NR time-frequency plane.}
	\label{fig:emBB_slots}
\end{figure}



The essence of the problem can be captured by comparing the two resource allocation configurations  shown in Figures~\ref{fig:config_1} and~\ref{fig:config_2}. In configuration~1,  eMBB user 1 is allocated the entire bandwidth for its aggregated slot duration. Let there be $ m_1 $ mini-slots in eMBB user 1's aggregated slot. Similarly  eMBB user 2 is allocated the entire bandwidth for its aggregated slot duration which consists of $ m_2 $ minislots.     The network state $s$ is assumed to be the same for the entire $ m_1 + m_2$ minislots. This implies that the loss functions of eMBB users $ (h_u^s\brac{\cdot}) $ do not change for $ m_1 + m_2 $ minislots. 

In Configuration~2  we shall allocate an eMBB user $ u $ a fraction $\phi_u$ of the bandwidth for a duration of $ m_1 + m_2 $ minislots, where $ \phi_u:=\frac{m_u}{m_1 +m_2} $ for $ u=1,2 $.  Note that the total resources allocated to eMBB users, which is the area allocated to them in the time-frequency plane is same in both these configurations.  In Configuration~1, the total puncturing observed by eMBB user $u$ is given by $\sum_{m=1}^{m_u} D(m) $.    In Configuration~2, under uniform URLLC placement, the total puncturing observed by eMBB user $u$ is given by $\sum_{m=1}^{m_1+m_2} \phi_u D(m)$. 
%Let us first define \emph{exchangeable} set of random variables. 
%\begin{definition}
%An ordered set of random variables $ \cbrac{D_1, D_2, \ldots, D_{\abs{\mathcal{M}}}}$ is said to be exchangeable if the probability distribution is same for any permutation of the set. 
%\end{definition}


The main result of this section is given below:
\begin{theorem}
	\label{thm:horizontal_vs_vertical}
Under the assumption of  i.i.d.  URLLC demands\footnote{This result can be extended to exchangeable URLLC demands. We use i.i.d. assumption to maintain consistency with other sections. } ($D(m), \, m=1,2, \ldots, m_1+m_2$)  and convex loss functions $(h_u^s \brac{\cdot})$,   for any eMBB user $ u $ we have that
\begin{equation}
\label{eq:result_on_vertical_vs_horizontal}
 \expect{h_u^s \brac{\sum_{m=1}^{m_u} D(m)}}  \geq \expect{h_u^s \brac{\sum_{m=1}^{m_1+m_2 } \phi_u D(m)}}.  
 \end{equation} 
\end{theorem}
Proof of this result is given in Appendix~\ref{pf:horizontal_vs_vertical}.


% \begin{proof}
% We can re-write R.H.S. of the above equations as follows:
% \begin{equation}
%  \expect{h_u \brac{\sum_{m=1}^{\abs{\mathcal{M} }} \phi_u D_m}} = \expect{h\brac{ \frac{1}{k+1} \sum_{q=1}^{k+1}\brac{\frac{\sum_{m \in \mathcal{M}\setminus q} D_m}{k}}}}.
% \end{equation}
% Using the above expression one can apply Jensen's inequality on the R.H.S. of~\eqref{eq:result_on_vertical_vs_horizontal}, we have that
% \begin{equation}
%\expect{h_u \brac{\sum_{m=1}^{\abs{\mathcal{M} }} \phi_u D_m}} \leq \frac{1}{k+1} \sum_{q=1}^{k+1} \expect{h_u\brac{\frac{\sum_{m \in \mathcal{M}\setminus q} D_m}{k}}}
% \end{equation}
% Since $D_m$'s are i.i.d., the R.H.S. of the above expression is same as the L.H.S. of~\eqref{eq:result_on_vertical_vs_horizontal}. Hence, proved. 
% \end{proof}
 {\em Remarks:} The above theorem shows that the expected  loss suffered by an eMBB user due to URLLC puncturing in  Configuration~1 is higher than in Configuration~2 during a coherence time.   This implies that all it is preferable for eMBB users to spread  their resource allocation in time  from the perspective of reducing their puncturing.  The underlying reason is that  Configuration~2  results in lesser variability in the total puncturing. Since the loss functions are convex, lower variability  leads to a lower expected loss. 
% Therefore, in any configuration  if eMBB users are allocated resources for different duration in an eMBB slot, then we can replace the configuration with an equivalent configuration which  allocates same amount of resources for all eMBB users but with same transmit duration and different bandwidths, while suffering  lower losses from puncturing by URLLC traffic.   
% 


 Now consider a more general configuration given in Fig.~\ref{fig:emBB_slots}. Suppose  we use a minislot homogeneous URLLC placement policy for the entire duration in Fig.~\ref{fig:emBB_slots}.   One can then apply the Thm.~\ref{thm:horizontal_vs_vertical} iteratively and show that using the same slot duration for eMBB users with appropriate scaling of the bandwidth allocation results in a higher average rate for eMBB users. 
% Therefore, for a common coherence time for all eMBB users, we shall use the same aggregated slot duration for all eMBB users with appropriate choice of bandwidth. Therefore, one can view a common coherence time as a `slot' for resource allocation to eMBB users, and hence, our system model which uses the same  slot duration for all users is justified. 
 \begin{figure}
\centering
\includegraphics[scale=0.33]{configuration_1}
\caption{In this configuration, eMBB users share time and do not share the bandwidth in an eMBB slot.}
\label{fig:config_1}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale=0.35]{configuration_2}
\caption{In this configuration, eMBB users share bandwidth and do not share the time in an eMBB slot.}
\label{fig:config_2}
\end{figure}


